Machine learning spectral functions in lattice QCD

We study the inverse problem of reconstructing spectral functions from Euclidean correlation functions via machine learning. We propose a novel neural network, SVAE, which is based on the variational autoencoder (VAE) and can be naturally applied to the inverse problem. The prominent feature of the SVAE is that a Shannon-Jaynes entropy term having the ground truth values of spectral functions as prior information is included in the loss function to be minimized. We train the network with general spectral functions produced from a Gaussian mixture model. As a test, we use correlators generated from four different types of physically motivated spectral functions made of one resonance peak, a continuum term and perturbative spectral function obtained using non-relativistic QCD. From the mock data test we find that the SVAE in most cases is comparable to the maximum entropy method (MEM) in the quality of reconstructing spectral functions and even outperforms the MEM in the case where the spectral function has sharp peaks with insufficient number of data points in the correlator. By applying to temporal correlation functions of charmonium in the pseudoscalar channel obtained in the quenched lattice QCD at 0.75 $T_c$ on $128^3\times96$ lattices and $1.5$ $T_c$ on $128^3\times48$ lattices, we find that the resonance peak of $\eta_c$ extracted from both the SVAE and MEM has a substantial dependence on the number of points in the temporal direction ($N_\tau$) adopted in the lattice simulation and $N_\tau$ larger than 48 is needed to resolve the fate of $\eta_c$ at 1.5 $T_c$.

==> Decoder.tikz.tex <==
\def\layersep{2.5cm}
\def\nodeinlayersep{1.5cm}
\resizebox{0.3\textwidth}{!}{%
\begin{tikzpicture}[
   shorten >=1pt,->,
   draw=black!50,
    node distance=\layersep,
    every pin edge/.style={<-,shorten <=1pt},
    neuron/.style={circle,fill=black!25,inner sep=0pt},
    input neuron/.style={neuron, fill=green!50, minimum size=35pt},
    output neuron/.style={neuron, fill=red!50, minimum size=35pt},
    hidden neuron/.style={neuron, fill=blue!50, minimum size=17pt},
    annot/.style={text width=4em, text centered}
]
    % Draw the input layer nodes
    \foreach \y/\Txt in {1/ \huge$z$}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
    \node[input neuron] (I-\y) at (0,-\y*4.5 cm) {\Txt};  %%% <-- MODIFIED
    % set number of hidden layers
    \newcommand\Nhidden{2}

    % Draw the hidden layer nodes
    \foreach \N in {1,...,\Nhidden} {
       \foreach \y in {1,...,5} { %%% MODIFIED (1,...,12 -> 1,...,5, and the next five lines)
         \ifnum \y=4
           \node at (\N*\layersep,-\y*\nodeinlayersep) {$\vdots$};
         \else
           \node[hidden neuron] (H\N-\y) at (\N*\layersep,-\y*\nodeinlayersep ) {};%write the inside mark
         \fi
       }
    \node[annot,above of=H\N-1, node distance=1cm] (hl\N) {Hidden layer \N};
    }
    % Draw the output layer node
    %\node[output neuron, right of=H\Nhidden-3] (O) {}; %%% <-- MODIFIED (from H\Nhidden-6 to H\Nhidden-3) 
        \foreach  \y/\Txt in {1/\Large$\rho(z)$,2/\Large$\alpha(z)$}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
              \node[output neuron] (o-\y) at (3*\layersep,-\y*3 cm) {\Txt};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1}
        \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
            \path (I-\source) edge (H1-\dest);
    % connect all hidden stuff
    \foreach [remember=\N as \lastN (initially 1)] \N in {2,...,\Nhidden}
       \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
           \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
               \path (H\lastN-\source) edge (H\N-\dest);
    % Connect every node in the hidden layer with the output layer
    %\foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
        %\path (H\Nhidden-\source) edge (O);
        \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
            \foreach \dest in {1,...,2}
               \path (H2-\source) edge (o-\dest);
    % Annotate the layers
    \node[annot,left of=hl1] {Input layer};
    \node[annot,right of=hl\Nhidden] {Output layer};
\end{tikzpicture}
}

==> Encoder1.tikz.tex <==
\def\layersep{2.5cm}
\def\nodeinlayersep{1.5cm}
\resizebox{0.3\textwidth}{!}{%
\begin{tikzpicture}[
   shorten >=1pt,->,
   draw=black!50,
    node distance=\layersep,
    every pin edge/.style={<-,shorten <=1pt},
    neuron/.style={circle,fill=black!25,inner sep=0pt},
    input neuron/.style={neuron, fill=green!50, minimum size=35pt},
    output neuron/.style={neuron, fill=red!50, minimum size=35pt},
    hidden neuron/.style={neuron, fill=blue!50, minimum size=17pt},
    annot/.style={text width=4em, text centered}
]
    % Draw the input layer nodes
    \foreach \y/\Txt in {1/ \huge$\rho_{gt}$,2/ \huge$G_{gt}$}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
    \node[input neuron] (I-\y) at (0,-\y*3 cm) {\Txt};  %%% <-- MODIFIED
    % set number of hidden layers
    \newcommand\Nhidden{2}

    % Draw the hidden layer nodes
    \foreach \N in {1,...,\Nhidden} {
       \foreach \y in {1,...,5} { %%% MODIFIED (1,...,12 -> 1,...,5, and the next five lines)
         \ifnum \y=4
           \node at (\N*\layersep,-\y*\nodeinlayersep) {$\vdots$};
         \else
           \node[hidden neuron] (H\N-\y) at (\N*\layersep,-\y*\nodeinlayersep ) {};%write the inside mark
         \fi
       }
    \node[annot,above of=H\N-1, node distance=1cm] (hl\N) {Hidden layer \N};
    }
    % Draw the output layer node
    %\node[output neuron, right of=H\Nhidden-3] (O) {}; %%% <-- MODIFIED (from H\Nhidden-6 to H\Nhidden-3) 
        \foreach  \y/\Txt in {1/\huge$\mu$,2/\huge$\sigma$,3/\huge$\pi$}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
              \node[output neuron] (o-\y) at (3*\layersep,-\y*2.2 cm) {\Txt};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,2}
        \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
            \path (I-\source) edge (H1-\dest);
    % connect all hidden stuff
    \foreach [remember=\N as \lastN (initially 1)] \N in {2,...,\Nhidden}
       \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
           \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
               \path (H\lastN-\source) edge (H\N-\dest);
    % Connect every node in the hidden layer with the output layer
    %\foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
        %\path (H\Nhidden-\source) edge (O);
        \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
            \foreach \dest in {1,...,3}
               \path (H2-\source) edge (o-\dest);
    % Annotate the layers
    \node[annot,left of=hl1] {Input layer};
    \node[annot,right of=hl\Nhidden] {Output layer};
\end{tikzpicture}
}

==> Encoder2.tikz.tex <==
\def\layersep{2.5cm}
\def\nodeinlayersep{1.5cm}
\resizebox{0.3\textwidth}{!}{%
\begin{tikzpicture}[
   shorten >=1pt,->,
   draw=black!50,
    node distance=\layersep,
    every pin edge/.style={<-,shorten <=1pt},
    neuron/.style={circle,fill=black!25,inner sep=0pt},
    input neuron/.style={neuron, fill=green!50, minimum size=35pt},
    output neuron/.style={neuron, fill=red!50, minimum size=35pt},
    hidden neuron/.style={neuron, fill=blue!50, minimum size=17pt},
    annot/.style={text width=4em, text centered}
]
    % Draw the input layer nodes
    \foreach \y/\Txt in {1/ \huge${G}$}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
    \node[input neuron] (I-\y) at (0,-\y*4.5 cm) {\Txt};  %%% <-- MODIFIED
    % set number of hidden layers
    \newcommand\Nhidden{2}

    % Draw the hidden layer nodes
    \foreach \N in {1,...,\Nhidden} {
       \foreach \y in {1,...,5} { %%% MODIFIED (1,...,12 -> 1,...,5, and the next five lines)
         \ifnum \y=4
           \node at (\N*\layersep,-\y*\nodeinlayersep) {$\vdots$};
         \else
           \node[hidden neuron] (H\N-\y) at (\N*\layersep,-\y*\nodeinlayersep ) {};%write the inside mark
         \fi
       }
    \node[annot,above of=H\N-1, node distance=1cm] (hl\N) {Hidden layer \N};
    }
    % Draw the output layer node
    %\node[output neuron, right of=H\Nhidden-3] (O) {}; %%% <-- MODIFIED (from H\Nhidden-6 to H\Nhidden-3) 
        \foreach  \y/\Txt in {1/\huge$\hat{\mu}$,2/\huge$\hat{\sigma}$,3/\huge$\hat{\pi}$}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
              \node[output neuron] (o-\y) at (3*\layersep,-\y*2.2 cm) {\Txt};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1}
        \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
            \path (I-\source) edge (H1-\dest);
    % connect all hidden stuff
    \foreach [remember=\N as \lastN (initially 1)] \N in {2,...,\Nhidden}
       \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
           \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
               \path (H\lastN-\source) edge (H\N-\dest);
    % Connect every node in the hidden layer with the output layer
    %\foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
        %\path (H\Nhidden-\source) edge (O);
        \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
            \foreach \dest in {1,...,3}
               \path (H2-\source) edge (o-\dest);
    % Annotate the layers
    \node[annot,left of=hl1] {Input layer};
    \node[annot,right of=hl\Nhidden] {Output layer};
\end{tikzpicture}
}

==> Flow1.tikz.tex <==
\usetikzlibrary{arrows.meta}
\usetikzlibrary{positioning,calc}
\tikzset{%
%  >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
      base/.style = {rectangle, rounded corners, draw=black,
                           minimum width=4cm, minimum height=1cm,
                           text centered, font=\sffamily},
       activityStarts/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=green!30},
       activityStarts1/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=red!30},
       KL/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2.5cm, minimum height=1.5cm,
                           text centered, font=\sffamily,fill=green!30},
    activityRuns/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=green!30},
         process/.style = {base, minimum width=2.5cm, fill=blue!15,
                           font=\ttfamily},
      functions/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=1cm,
                           text centered, font=\sffamily, fill=yellow!30},
}
\def\layersep{2.5cm}
\def\nodeinlayersep{1.5cm}
\resizebox{1\textwidth}{!}{% 
\begin{tikzpicture}[node distance=2cm,
    every node/.style={fill=white, font=\sffamily}, align=center]
  % Specification of nodes (position, etc.)
  \coordinate (input);
  \node (PG)             [activityStarts]              {$G_{gt}$\\ $\rho_{gt}$};
  \node (Encoder1)     [process, right= 5mm of PG]          {Encoder 1};
%  \node (es1)      [activityStarts1,  right= 5mm of Encoder1]   {$\mu$, $\sigma$,\\$\pi$};
  \node (es1)      [activityStarts1,  right= 5mm of Encoder1]   {$Q(z|G_{gt},\rho_{gt})$};
   \node (Ghat)     [activityStarts, below of=PG]   {${G}$};
    \node (Encoder2)     [process, right of=Ghat]          {Encoder 2};
    \node (es2)      [activityStarts1, right= 5mm of Encoder2]   {$P(z|{G})$};
 %  \node (onResumeBlock)     [activityStarts, right of =es1]   {z\\z\\z\\z\\z};
%   \node (onResumeBlock)  [KL, right= 2 cm of {$(es1)!0.5!(es2)$}]   {\huge{$z$}\\(K-L divergence)}; 
   %\node (onResumeBlock)  [activityRuns, minimum height=1cm, right= 2 cm of {$(es1)!0.5!(es2)$}]  {sampling \large{$z$}}; 
   \node (onResumeBlock)  [activityRuns, minimum height=1cm, right= 5 mm of es1]  {sampling \large{$z$}}; 
      \node (Decoder)     [process, right= 5mm of onResumeBlock]   {Decoder};
        \node (alphaG)     [activityStarts, right= 5mm of Decoder]   {$\rho(z)\to G[\rho(z)]$\\$\alpha(z)$};
       %\node [activityStarts] at ($(Decoder.north east)!.5!(alphaG.north west)$) (rhoz) {$\rho(z)$}      
      % \node (es3)      [activityStarts1, right of=Decoder]   {$\mu$\\ $\sigma$};
      \node (KL)  [functions,   right=3.5 cm of es2]   {$KL$ divergence};
      \node (E)     [functions, right=5mm of alphaG]   {$E_{Q}[\log P(\rho|z, {G})]$};
       \node (lossfun)     [ functions, below of= E]   {Loss function};
      % \node (rhoz)     [activityStarts, above left = 2mm of E]   {$\rho(z)$};
   % Specification of lines between nodes specified above
  % with aditional nodes for description 
    \draw[->]             (PG) -- (Encoder1);
    \draw[->]             (Encoder1) -- (es1);
%    \draw[->]             (es1) -- node[xshift=-0.6cm, yshift=-0.65cm,text width=0.2cm]{sampling}(onResumeBlock);
    \draw[->]             (es1) -- (onResumeBlock);
    \draw[->]             (onResumeBlock) -- (Decoder);
      \draw[->]             (Ghat) -- (Encoder2);
      \draw[->]             (Encoder2) -- (es2);
       \draw[->]             (es2) -- (KL);
       \draw[->]             (alphaG) -- (E);      
       \draw[->]              (Decoder) -- (alphaG);
         \draw[->]             (E) -- (lossfun);
         \draw[->]             (KL) -- (lossfun); 
          \draw[->]             ([yshift=-5mm] es1.east) -- (KL);
  \end{tikzpicture}
  }
  
  

==> Flow2.tikz.tex <==
%\usetikzlibrary{arrows.meta}
%\usetikzlibrary{positioning,calc}

\tikzset{%
%  >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
      base/.style = {rectangle, rounded corners, draw=black,
                           minimum width=4cm, minimum height=1cm,
                           text centered, font=\sffamily},
       activityStarts/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=1cm,
                           text centered, font=\sffamily, fill=green!30},
       activityStarts1/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=red!30},
       KL/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2.5cm, minimum height=1.5cm,
                           text centered, font=\sffamily,fill=green!30},
    activityRuns/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=green!30},
         process/.style = {base, minimum width=2.5cm, fill=blue!15,
                           font=\ttfamily},
}
\def\layersep{2.5cm}
\def\nodeinlayersep{1.5cm}
%\resizebox{0.35\textwidth}{!}{% 
\begin{tikzpicture}[node distance=2cm,
    every node/.style={fill=white, font=\sffamily}, align=center]
  % Specification of nodes (position, etc.)
  \coordinate (input);
   \node (Ghat)     [activityRuns, below of=PG]   {${G}$};
    \node (Encoder2)     [process, right of=Ghat]          {Encoder 2};
    \node (es2)      [activityStarts1, right=6mm, at=(Encoder2.east)]   {$P(z|{G})$};
 %  \node (onResumeBlock)     [activityStarts, right of =es1]   {z\\z\\z\\z\\z};
 %  \node (onResumeBlock)  [activityRuns, right of = es2]   {$z$}; 
   \node (onResumeBlock)  [activityRuns, minimum height=1cm, right=6mm, at=(es2.east)]   {sampling \large{$z$}}; 
      \node (Decoder) [process, right=6mm,at=(onResumeBlock.east)]   {Decoder};
     %  \node (es3)      [activityStarts1, right of=Deconder]   {$\mu$\\ $\sigma$};
      \node (rho)     [activityRuns, minimum height=1cm, right=6mm, at=(Decoder.east)]   { $\rho(z)$\\$\alpha(z)$};
  % Specification of lines between nodes specified above
  % with aditional nodes for description 
    \draw[->]             (onResumeBlock) -- (Decoder);
      \draw[->]             (Ghat) -- (Encoder2);
      \draw[->]             (Encoder2) -- (es2);
%       \draw[->]             (es2) --  node[xshift=-0.5cm, yshift=0.3cm,text width=0.2cm]{sampling}(onResumeBlock);
       \draw[->]             (es2) --  node[xshift=0cm, yshift=0.3cm,text width=0cm]{}(onResumeBlock);
        \draw[->]             (Decoder) -- (rho);
       % \draw[->]             (es3) -- node[xshift=-0.5cm, yshift=0.3cm,text width=0.2cm]{sampling}(rho);
     %  \draw[->]            (es3)--(rho);
  \end{tikzpicture}
 % }
 
  
